Tensor-based Emotion Editing in the StyleGAN Latent Space

In this paper, we use a tensor model based on the Higher-Order Singular Value Decomposition (HOSVD) to discover semantic directions in Generative Adversarial Networks. This is achieved by first embedding a structured facial expression database into the latent space using the e4e encoder. Specifically, we discover directions in latent space corresponding to the six prototypical emotions: anger, disgust, fear, happiness, sadness, and surprise, as well as a direction for yaw rotation. These latent space directions are employed to change the expression or yaw rotation of real face images. We compare our found directions to similar directions found by two other methods. The results show that the visual quality of the resultant edits are on par with State-of-the-Art. It can also be concluded that the tensor-based model is well suited for emotion and yaw editing, i.e., that the emotion or yaw rotation of a novel face image can be robustly changed without a significant effect on identity or other attributes in the images.

==> sec/discussion.tex <==
\section{Conclusion}
% What have we done
In this work, we have presented an extension of the HOSVD-based tensor model, proposed in \cite{Haas2021tensorGAN}.
% for the StyleGAN latent space. 
In contrast to \cite{Haas2021tensorGAN}, (1) we use the e4e encoder \cite{Tov2021e4e} to recover highly editable latent codes for the BU-3DFE database, (2) we improve reconstruction in the tensor model by allowing the parameters to be full-rank, and (3) we show that edits can be applied directly in latent space.
% circumventing the need for for recovering the tensor model parameters prior to editing a latent code. 
% $\mathcal{W+}$ space without the need for prior recovery of the tensor model parameters. %
% Comparing to FG 
% We found that it is possible to make better reconstructions of novel images by utilizing a parameter tensor representation for the model rather than multiple parameter vectors, i.e., by relaxing the implicit rank-one constraint.
% in the original model, thus the stacked style-separated tensor model which was proposed proposed as an extension in \cite{Haas2021tensorGAN} is unnecessary. 
Further, we showed that we can calculate linear directions in  latent space corresponding to the six prototypical emotions by truncating the emotion intensity subspace.
% A limitation of the tensor model is that it requires balanced data, i.e. each expression and rotation must be performed by each person, which we plan to address in future work. 
%
After obtaining a latent representation of the data, constructing the tensor model is fast, requiring only a few minutes to calculate the HOSVD.
%
Further, the latent space directions corresponding to the six prototypical emotions can be calculated from the tensor model and subsequently applied to any latent code in the original latent space without the need to first estimate the subspace parameters  as otherwise suggested in \cite{Haas2021tensorGAN}. In other words, the found semantic directions are global and can be applied to any latent code without any further calculations. 
%
%
% Sum up
Our method is able to identify directions in latent space corresponding to yaw rotation, as well as each of the six basic expressions. 
The quality of the edits performed with these directions is on par with the corresponding edits using GANSpace \cite{Harkonen2020GANSpace} and InterFaceGAN \cite{Shen2020InterfaceganTPAMI}. 
%


% We found that recovering the tensor model parameters for a latent code is not strictly necessary for emotion editing as otherwise suggested in \cite{Haas2021tensorGAN}, which simplifies the editing procedure.

%
% Furthermore, the estimated latent codes were stable in rotation transfer, unlike the images corresponding to the non-regularized parameter vectors reported \cite{Haas2021tensorGAN}. 
% The more editable latent codes were obtained by using the e4e encoder \cite{Tov2021e4e}, rather than the ResNet initialization with VGG fine-tuning method for GAN inversion which was used in the previous work.
%

% A limitation of the tensor model is the requirement that for each person, all emotions and rotations must be available without any missing data. We plan to address this limitation in future work. 


% It is worth mentioning that we do not experience that the latent codes explode in magnitude when performing rotation transfer with  latent codes represented with non-regularised parameter vectors as reported in \cite{Haas2021tensorGAN}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% \red{Although the tensor model with full-rank a parameter tensor lowers the reconstruction error, it is unclear how we can edit the parameter tensor.}
% each of the expressions are available. 
% Data sets with this complete structure are 
% [mention limitation, bu3dfe structure]

% \begin{itemize}
% \item \red{Ideas}
% \item Comparing smile/happy direction is a difficult problem. 
% \item  
% \item 2d / 3d zooming effect. 
% \end{itemize}

